Scanning Trojaned Models Using Out-of-Distribution Samples

Scanning for trojan (backdoor) in deep neural networks is crucial due to their significant real-world applications. There has been an increasing focus on developing effective general trojan scanning methods across various trojan attacks. Despite advancements, there remains a shortage of methods that perform effectively without preconceived assumptions about the backdoor attack method. Additionally, we have observed that current methods struggle to identify classifiers trojaned using adversarial training. Motivated by these challenges, our study introduces a novel scanning method named TRODO (TROjan scanning by Detection of adversarial shifts in Out-of-distribution samples). TRODO leverages the concept of "blind spots"--regions where trojaned classifiers erroneously identify out-of-distribution (OOD) samples as in-distribution (ID). We scan for these blind spots by adversarially shifting OOD samples towards in-distribution. The increased likelihood of perturbed OOD samples being classified as ID serves as a signature for trojan detection. TRODO is both trojan and label mapping agnostic, effective even against adversarially trained trojaned classifiers. It is applicable even in scenarios where training data is absent, demonstrating high accuracy and adaptability across various scenarios and datasets, highlighting its potential as a robust trojan scanning strategy.

==> Dump/badnetvsothers.tex <==
\begin{figure*}[h]
    \label{badandother}
  \begin{center}
    \includegraphics[width=1\linewidth]{Images/badnetvsothers.pdf}
    \caption{Comparison of Accuracy across different trojan scanning methods. The chart illustrates the performance of each method on BadNet (orange) versus all other attacks (blue) in our collection of 8 distinct attack methods. Notably, our method (TRODO) maintains a consistent performance across both BadNet and other attacks. This indicates a superior generalization capability compared to other \kian{(attack or scanning?)} methods, which display a marked preference and possible overfitting to BadNet, leading to reduced scanning ability on varied attack types. \kian{There is no ref to Fig 2 in the text. Also, why did you choose Badnet separate from all other methods? The conclusion written about this figure is also unclear.}}
    
    \vspace*{-4mm}
    \label{fig:motivate_fig}
  \end{center}
\end{figure*}

==> Sec/Theory.tex <==
% \section{Theory}



% Train loss
% \begin{equation}
% \hat{\theta}=\underset{\theta}{\operatorname{argmin}} \frac{1}{n} \sum^{n}_{i=1} \mathcal{L}\left(f_\theta\left(x_i\right), y_i\right)
% \end{equation}

% Test loss
% \begin{equation}
% \frac{1}{m} \sum_{i=1}^m \mathcal{L}\left(f_{\hat{\theta}}\left(x_i^{\prime}\right), y_i^{\prime}\right) \approx \epsilon
% \leftarrow{\left\|\theta_0-\hat{\theta}\right\|_2} \approx \eta
% \end{equation}

% Train adv loss
% \begin{equation}
% \hat{\delta}=\underset{\delta \in \Delta}{\operatorname{argmax}}
% \overbrace{\mathcal{L}\left(f_\theta(x+\delta), y\right)}^M
% \end{equation}

% \begin{equation}
% x^{\prime} \approx x, 
% \mathcal{L}\left(f_{\hat{\theta}}\left(x^{\prime}+\hat{\delta}\right), y\right) \approx M
% \leftarrow{\left\|\delta_0-\hat{\delta}\right\|_2}
% \end{equation}

% Module Criticality
% \begin{equation}
% G G \propto \sqrt{\frac{\sum_{i=0}\log \left(1+M C_i\right)+\cdots}{m-1}}
% \end{equation}





==> Tables/adaptive_attack.tex <==
\begin{table}[h]
\centering
\small % Adjust font size

\caption{Accuracy of our method with different loss functions under adaptive attacks.}
\label{tab:adaptive_loss}
\renewcommand{\arraystretch}{1.5}\setlength{\tabcolsep}{10pt} % Adjust row height and column spacing
\resizebox{1\linewidth}{!}{%
\begin{tabular}{l l c c c c c c c}

\specialrule{3pt}{\aboverulesep}{\belowrulesep}

\textbf{Label Mapping} & \textbf{Loss} & \textbf{MNIST} & \textbf{CIFAR10} & \textbf{GTSRB} & \textbf{CIFAR100} & \textbf{PubFig} & \textbf{Avg.} \\

\specialrule{3pt}{\aboverulesep}{\belowrulesep}

\multirow{3}{*}{All-to-One} 
& $L_{\text{default}}$ & 91.2 / 89.6 & 91.0 / 88.4 & 96.6 / 93.2 & 86.7 / 82.5 & 88.1 / 83.0 & 90.7 / 87.3 \\ 
& $L_{\text{adaptive1}}$ & 87.3 / 86.3 & 88.1 / 86.6 & 93.0 / 90.8 & 83.3 / 81.0 & 83.7 / 81.1 & 87.1 / 85.2 \\ 
& $L_{\text{adaptive2}}$ & 87.1 / 84.8 & 87.1 / 84.5 & 91.7 / 89.2 & 79.8 / 78.5 & 81.0 / 79.8 & 85.3 / 83.4 \\ 

\cmidrule(lr){1-8}

\multirow{3}{*}{All-to-All} 
& $L_{\text{default}}$ & 90.0 / 87.4 & 89.3 / 87.5 & 92.6 / 89.1 & 82.4 / 85.0 & 83.2 / 80.9 & 87.5 / 86.0 \\ 
& $L_{\text{adaptive1}}$ & 84.4 / 83.3 & 85.5 / 83.8 & 85.6 / 84.1 & 78.5 / 77.3 & 79.7 / 77.8 & 82.7 / 81.4 \\ 
& $L_{\text{adaptive2}}$ & 76.9 / 74.8 & 78.2 / 76.8 & 82.1 / 80.4 & 73.0 / 71.3 & 69.2 / 67.0 & 75.9 / 74.1 \\ 

\specialrule{3pt}{\aboverulesep}{\belowrulesep}

\end{tabular}%
}
\end{table}


==> Tables/app_preact.tex <==
\begin{table}[h]
\centering
\small % Adjust font size
\centering
\caption{Performance of TRODO compared with other methods, in terms of Accuracy (ACC \%) and AUROC (AUC \%). The best results are emphasized in \textbf{bold} format respectively in each column.}
% Performance evaluation of our model against various advanced adversarial attacks, measured by AUC (\%), with $\epsilon=\frac{4}{255}$ for low-resolution images and $\epsilon=\frac{2}{255}$ for high-resolution images, Measured by AUC (\%). The best results are emphasized in bold format respectively in each row. The table cells denote results in the "PGD/\graytext{Clean}" format.

\label{tab:preact_results}
\renewcommand{\arraystretch}{1}\setlength{\tabcolsep}{4pt} \Large % Adjust row height
% \resizebox{0.6\linewidth}{!}{\begin{tabular}{lcccccc}
    \resizebox{1\linewidth}{!}{\begin{tabular}{c*{12}{C{2cm}}} 

    % \noalign{\smallskip}\hline\noalign{\smallskip}
     \specialrule{3pt}{\aboverulesep}{\belowrulesep}

     \multirow{2}{*}{Method}  & \multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{MNIST} &  \multicolumn{2}{c}{GTSRB} & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{Pubfig} & \multicolumn{2}{c}{\textbf{AVG}} \\
    
     \cmidrule(lr){2-3}   \cmidrule(lr){4-5} \cmidrule{6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
     
    
   & AUC & ACC & AUC & ACC & AUC & ACC  & AUC & ACC & AUC & ACC & \textbf{AUC} & \textbf{ACC}\\   

     \specialrule{3pt}{\aboverulesep}{\belowrulesep}

      NC & X & X & X & X & X & X & X & X & X & X & X & X\\
             \cmidrule(lr){1-13}

      ULP & X & X & X & X & X & X & X & X & X & X & X & X\\
        \cmidrule(lr){1-13}

     ABS & X & X & X & X & X & X & X & X & X & X & X & X\\
             \cmidrule(lr){1-13}

     K-Arm & X & X & X & X & X & X & X & X & X & X & X & X\\
        \cmidrule(lr){1-13}

    UMD & X & X & X & X & X & X & X & X & X & X & X & X\\
         \cmidrule(lr){1-13}

     TOPO & X & X & X & X & X & X & X & X & X & X & X & X\\
        \cmidrule(lr){1-13}
     \textbf{TRODO (Ours)} & 91.0 & 87.6 & 91.2 & 89.6 & 96.6 & 89.1 & 88.7 & 85 & - & - & - & -\\
     
     \specialrule{3pt}{\aboverulesep}{\belowrulesep}
\end{tabular}}
\end{table}

% \vspace{-20pt}



